Thermorefringent noise in crystalline optical materials

Any material in thermal equilibrium exhibits fundamental thermodynamic fluctuations of its mechanical and optical properties. Such thermodynamic fluctuations of length, elastic constants, and refractive index of amorphous materials -- like dielectric mirror coatings and substrates -- limit the performance of today's most precise optical instruments. Crystalline materials are increasingly employed in optical systems because of their reduced mechanical dissipation, which implies a reduction of thermo-mechanical fluctuations. However, the anisotropy of the crystalline state implies a fundamental source of thermal noise: depolarization induced by thermal fluctuations of its birefringence. We establish the theory of this effect, elucidate its consequences, discuss its relevance for precision optical experiments with crystalline materials, and hint at the conditions under which it can be evaded.

==> readout.tex <==
\section{Implications for optical detection}
\label{sec:readout}

One can estimate the polarization angle noise associated with the
transmission through the material. In general, the outgoing light beam
will have elliptical polarization. However, characteristics strength of the
field along $x$ is much stronger than $y$ due to a presence of strong
incoming field with $x$ polarization. One can estimate the magnitude
of polarization deviaion using the following formula:
\begin{equation}	\label{eq:angle_deviation}
	\delta \Theta \simeq \frac{|\delta E_y|}{|E_x|}.
\end{equation}
\edh{We expect $\delta\Theta$ to fluctuate around both sides of zero, so I am suspicious of the absolute value sign in the numerator.}
Therefore, one can write the correlation function for $\delta \Theta$ as in
\begin{equation} \label{eq:angle_noise}
	\avg{\delta \Theta(t) \, \delta \Theta(t + \tau)} \simeq \frac{1}{P} \avg{|\delta E_y (t)| \, |\delta E_y (t + \tau)|}
\end{equation}
The correlation function in \cref{eq:angle_noise} has a similar structure
to a correlation function for $E_x$. The only difference is the absence of the complex
exponential term of the form $e^{i k c \tau}$. The power spectral density for the 
polarization angle $S_{\Theta \Theta} (\Omega)$
will have a very similar structure: the absence of the exponent will shift $S_{xx}(\Omega)$
to $S_{xx}(\Omega - kc)$.
Therefore,
\begin{equation}
	S_{\Theta \Theta}(\Omega) = \frac{1}{P} S_{xx}(\Omega - kc).
\end{equation}
For the values of frequency $\Omega \ll ck$, \cref{eq:S_yy_asympt_inf1}
yields
\begin{equation}
	S_{\Theta \Theta}(\Omega) = \frac{|\eps_{yx}'|^2 k_B T^2 \ell}{2 \pi r_0^2 n_y^2 (n_x - n_y)^2 D_{zz} c_V }.
    \label{eq:ThetaPSD}
\end{equation}
Noise in polarization angle has a white noise profile for the low frequencies.

\vs{STOKES PARAMETERS}

\subsection{Direct photodetection}

\subsection{Homodyne detection}

\edh{expand to include dc readout and polarimetry readout}

We now turn to the question of how the thermorefringent noise in
\cref{eq:ThetaPSD} manifests in a typical homodyne detection scheme, as might
be desired to read out some phase signal impressed on the signal light.
Collecting the signal amplitudes $E_x$ and $E_y$ into a phasor $\mathbf{E}$, the
electric field emerging from the crystal material has the Jones matrix
\begin{equation}
    \mathbf{E} = \begin{pmatrix}
        \cos{\Theta(t)} \rme^{\rmi\Phi_x(t)} \\
        \sin{\Theta(t)} \rme^{\rmi\Phi_y(t)}
    \end{pmatrix} \rme^{\rmi\omega t} + \text{cc},
\end{equation}
where $\Theta(t)$ is the time-varying polarization angle of the resultant
signal light, which has a fluctuating part given by \cref{eq:ThetaPSD}, and
could additionally have a static misalignment $\Theta_0$.  $\Phi_{x,y}(t)$ are
fluctuating phase terms for the $x$ and $y$ components of the light. \edh{Need
to check that \cref{eq:ThetaPSD} is still valid if the light entering the
crystal already has $x$ and $y$ components.}

If this signal is beaten against local oscillator (LO) light, with Jones matrix
\begin{equation}
    \mathbf{E}_\text{LO} = \begin{pmatrix}
        \cos{\Theta_\text{LO}} \\
        \sin{\Theta_\text{LO}} 
    \end{pmatrix} \rme^{\rmi\Phi_\text{LO}} \rme^{\rmi\omega t} + \text{cc},
\end{equation}
where $\Theta_\text{LO}$ and $\Phi_\text{LO}$ are the (static) polarization and
phase angles, respectively, then the resulting photocurrent $I \propto |\mathbf{E}_\text{LO}^* \cdot \mathbf{E}|$ is
\begin{multline}
    I \propto \cos{\Theta(t)} \cos{\Theta_\text{LO}} \cos[\Phi_x(t) - \Phi_\text{LO}] \\
        + \sin{\Theta(t)} \sin{\Theta_\text{LO}} \cos[\Phi_y(t) - \Phi_\text{LO}].
\end{multline}
Suppose that the phase signal of interest is the fluctuating part of $\Phi_x(t) \equiv \langle\Phi_x\rangle + \phi_x(t)$. To perform a homodyne readout of this phase, we
should choose $\Phi_\text{LO} = \langle\Phi_x\rangle + \pi/2$. Assuming that the fluctuations
$\phi_{x,y}(t)$ are small, then
\begin{multline}
    I \propto (\cos{\Theta(t)} \cos{\Theta_\text{LO}}) \phi_x(t) \\
        + \sin{\Theta(t)} \sin{\Theta_\text{LO}} [\sin\Delta\Phi + \phi_y(t) \cos\Delta\Phi],
\end{multline}
where $\Delta\Phi = \langle\Phi_y\rangle - \langle\Phi_x\rangle$.
Now writing $\Theta(t) = \langle\Theta\rangle + \theta(t)$, with $\theta(t)$ small, we find
\begin{multline}
    I \propto  (\cos{\Theta_\text{LO}}\cos{\langle\Theta\rangle}) \phi_x(t)
        + \sin{\Theta_\text{LO}}[\sin{\langle\Theta\rangle}\sin\Delta\Phi \\
        + (\sin{\langle\Theta\rangle}\cos{\Delta\Phi}) \phi_y(t)
        + (\cos{\langle\Theta\rangle}\sin{\Delta\Phi}) \theta(t)].
\end{multline}
We see that compared to the phase signal of interest $\phi_x$, the polarization noise $\theta$ enters with a relative factor $\tan\Theta_\text{LO} \sin\Delta\Phi$.

\edh{Insert some summing-up words here about the (ir)reducibility of these noises.}

\subsection{Polarimetry}

